Generative Visual Foresight Meets Task-Agnostic Pose Estimation in Robotic Table-Top Manipulation

Robotic manipulation in unstructured environments requires systems that can generalize across diverse tasks while maintaining robust and reliable performance. We introduce {GVF-TAPE}, a closed-loop framework that combines generative visual foresight with task-agnostic pose estimation to enable scalable robotic manipulation. GVF-TAPE employs a generative video model to predict future RGB-D frames from a single side-view RGB image and a task description, offering visual plans that guide robot actions. A decoupled pose estimation model then extracts end-effector poses from the predicted frames, translating them into executable commands via low-level controllers. By iteratively integrating video foresight and pose estimation in a closed loop, GVF-TAPE achieves real-time, adaptive manipulation across a broad range of tasks. Extensive experiments in both simulation and real-world settings demonstrate that our approach reduces reliance on task-specific action data and generalizes effectively, providing a practical and scalable solution for intelligent robotic systems.

==> images/tex/act_h.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{images/act_h_sr.pdf}
    \caption{
    \textbf{Success rate across LIBERO-Spatial with different action horizons.} Shorter horizons are more prone to illusion, while longer ones provide stability.
    }
    \label{fig:act_h}
    \vspace{-2mm}
\end{figure}

==> images/tex/ddim_flow.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{images/DDIM_vs_RF.pdf}
       
    
    \caption{\small
    \textbf{Generation quality comparison of diffusion and rectified flow.} More sampling timesteps improve diffusion-based methods but increase inference time. Rectified flow achieves strong performance with only three steps.
    }
    \label{fig:ddim_flow}
\end{figure}

==> images/tex/huamn_hand.tex <==
\begin{figure}[t]
    \vspace{2mm}
    \centering
    \includegraphics[width=0.98\linewidth]{images/huamn_hand_v2.png}
    \caption{\small
    \textbf{A comparison between human and robotic manipulation.} (a) and (b) illustrate how humans, with experience in manipulation, can easily imagine the desired hand pose at a simple glance. GVF-TAPE aims to replicate this ability in table-top robotic manipulation scenarios.
    }
    \label{fig:human_hand}
    \vspace{-4mm}
\end{figure}


==> images/tex/intro_lb.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth, trim={2.1cm 5.6cm 3.3cm 5.0cm},clip]{images/intro_lb.pdf}
    \caption{An overview of LIBERO dataset}
    \linfang{@Chuye @Xiaoxiong: Consider move this figure to Supplementary, and put a move valuable experiment figure to the main paper.}
    \label{fig:intro_lb}
\end{figure}

==> images/tex/real_sc.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-5mm} % adjust vertical spacing as needed
    \centering
    \includegraphics[width=0.48\textwidth]{images/real_world_success_rates_v5.png}
    \caption{Success rates over different real world tasks.}
    \label{fig:real_sc}
    \vspace{-3mm}
\end{wrapfigure}


==> images/tex/success_tasks.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/success_sponge.png}
    \caption{Completing Task: put the sponge on the red plate. The upper row is generated key video frames and the the next row below consists of corresponding robot action in real world}
    \label{fig:success_sponge}
\end{figure*}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/red_success.png}
    \caption{Completing Task: put the red cup on the silver plate. The upper row is generated key video frames and the next row below consists of corresponding robot action in real world}
    \label{fig:red_success}
\end{figure*}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/banana_success.png}
    \caption{Completing Task:pick up the banana and place it in the basket. The upper row is generated key video frames and the next row below consists of corresponding robot action in real world}
    \label{fig:red_success}
\end{figure*}
